Early Failure Detection in Autonomous Surgical Soft-Tissue Manipulation via Uncertainty Quantification

Autonomous surgical robots are a promising solution to the increasing demand for surgery amid a shortage of surgeons. Recent work has proposed learning-based approaches for the autonomous manipulation of soft tissue. However, due to variability in tissue geometries and stiffnesses, these methods do not always perform optimally, especially in out-of-distribution settings. We propose, develop, and test the first application of uncertainty quantification to learned surgical soft-tissue manipulation policies as an early identification system for task failures. We analyze two different methods of uncertainty quantification, deep ensembles and Monte Carlo dropout, and find that deep ensembles provide a stronger signal of future task success or failure. We validate our approach using the physical daVinci Research Kit (dVRK) surgical robot to perform physical soft-tissue manipulation. We show that we are able to successfully detect out-of-distribution states leading to task failure and request human intervention when necessary while still enabling autonomous manipulation when possible. Our learned tissue manipulation policy with uncertainty-based early failure detection achieves a zero-shot sim2real performance improvement of 47.5% over the prior state of the art in learned soft-tissue manipulation. We also show that our method generalizes well to new types of tissue as well as to a bimanual soft-tissue manipulation task.

==> intro-fig.tex <==
\setcounter{figure}{1}
\makeatletter
\let\@oldmaketitle\@maketitle
\renewcommand{\@maketitle}{\@oldmaketitle \begin{center} \centering \includegraphics[width=1.0\textwidth]{MainFigFlat.png}  \vspace{-18pt}\label{fig:intro-fig}\end{center}\footnotesize{\textbf{Fig.~\thefigure:\label{fig:sequence1}~Overall pipeline and experimental setup.} We sense a point cloud of the current geometry of the tissue using the Segment Anything Model (SAM)~\citep{kirillov2023segment} to segment RGBD images of the scene. SAM takes as input the RGB components of the image along with a query point on the desired segmented object. The resulting segmentation mask is then converted into a point cloud using the depth component of the image along with the camera's intrinsic matrix to give the three-dimensional geometry of the tissue. The current geometry, coupled with the goal geometry and manipulation point, are passed as input to a deep ensemble of DeformerNet~\citep{thach2023deformernet} models to predict a robot action $\hat{\mathrm{A}}$ (homogeneous transformation matrix) and an uncertainty estimate $u$. Using $u$, we determine if it is safe for the daVinci Research Kit (dVRK) robot to take action $\hat{\mathrm{A}}$. If yes, the robot takes action $\hat{\mathrm{A}}$, and the process repeats. Otherwise, the system requests a human to intervene and complete the task. We perform human interventions using the surgeon-side dVRK manipulators for teleoperation.}\vspace{-18pt}\medskip}
\makeatother
\maketitle
